UAV Tracking with Solid-State Lidars:Dynamic Multi-Frequency Scan Integration

With the increasing use of drones across various industries, the navigation and tracking of these unmanned aerial vehicles (UAVs) in challenging environments (such as GNSS-denied environments) have become critical issues. In this paper, we propose a novel method for a ground-based UAV tracking system using a solid-state LiDAR, which dynamically adjusts the LiDAR frame integration time based on the distance to the UAV and its speed. Our method fuses two simultaneous scan integration frequencies for high accuracy and persistent tracking, enabling reliable estimates of the UAV state even in challenging scenarios. The use of the Inverse Covariance Intersection method and Kalman filters allow for better tracking accuracy and can handle challenging tracking scenarios. We have performed a number of experiments for evaluating the performance of the proposed tracking system and identifying its limitations. Our experimental results demonstrate that the proposed method achieves comparable tracking performance to the established baseline method, while also providing more reliable and accurate tracking when only one of the frequencies is available or unreliable.

==> tex/ape_boxplot_adaptive_circ_traj.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

  \definecolor{darkslategray38}{RGB}{38,38,38}
  \definecolor{lavender234234242}{RGB}{234,234,242}
  \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
  \definecolor{steelblue76114176}{RGB}{76,114,176}

  \begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    axis background/.style={fill=white},
    axis line style={white},
    tick align=outside,
    x grid style={white},
    xmajorgrids,
    xmajorticks=true,
    xmin=0.5, xmax=6.5,
    xtick style={draw=none},
    xtick={1,2,3,4,5,6},
    xticklabels={
      \(\displaystyle I_{}^{\text{KF}}\),
      \(\displaystyle I_{\text{AST}}^{\text{KF}}\),
      \(\displaystyle I_{\text{ADT}}^{\text{KF}}\),
      \(\displaystyle I_{}^{\text{EKF}}\),
      \(\displaystyle I_{\text{AST}}^{\text{EKF}}\),
      \(\displaystyle I_{\text{ADT}}^{\text{EKF}}\)
    },
    y grid style={white},
    ylabel=\textcolor{darkslategray38}{Error (m)},
    ymajorgrids,
    ymajorticks=true,
    ymin=-0.0186402966221774, ymax=0.0964276981289192,
    % ytick style={draw=none}
    % ytick style={draw=none}
    y grid style={white!69.0196078431373!black},
    ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
    ]
    \path [draw=color2, fill=color2]
    (axis cs:0.75,0.00715694641221769)
    --(axis cs:1.25,0.00715694641221769)
    --(axis cs:1.25,0.0308042346226179)
    --(axis cs:0.75,0.0308042346226179)
    --(axis cs:0.75,0.00715694641221769)
    --cycle;
    \addplot [black]
    table {%
    1 0.00715694641221769
    1 -0.0134099332244002
    };
    \addplot [black]
    table {%
    1 0.0308042346226179
    1 0.0543099492747481
    };
    \addplot [black]
    table {%
    0.875 -0.0134099332244002
    1.125 -0.0134099332244002
    };
    \addplot [black]
    table {%
    0.875 0.0543099492747481
    1.125 0.0543099492747481
    };
    \path [draw=color2, fill=color2]
    (axis cs:1.75,0.00464528547541216)
    --(axis cs:2.25,0.00464528547541216)
    --(axis cs:2.25,0.0226626725793369)
    --(axis cs:1.75,0.0226626725793369)
    --(axis cs:1.75,0.00464528547541216)
    --cycle;
    \addplot [black]
    table {%
    2 0.00464528547541216
    2 -0.0126850896982031
    };
    \addplot [black]
    table {%
    2 0.0226626725793369
    2 0.040433099008579
    };
    \addplot [black]
    table {%
    1.875 -0.0126850896982031
    2.125 -0.0126850896982031
    };
    \addplot [black]
    table {%
    1.875 0.040433099008579
    2.125 0.040433099008579
    };
    \path [draw=color2, fill=color2]
    (axis cs:2.75,0.0126176652881678)
    --(axis cs:3.25,0.0126176652881678)
    --(axis cs:3.25,0.0389424754339975)
    --(axis cs:2.75,0.0389424754339975)
    --(axis cs:2.75,0.0126176652881678)
    --cycle;
    \addplot [black]
    table {%
    3 0.0126176652881678
    3 -0.0105623738165284
    };
    \addplot [black]
    table {%
    3 0.0389424754339975
    3 0.0652578713470367
    };
    \addplot [black]
    table {%
    2.875 -0.0105623738165284
    3.125 -0.0105623738165284
    };
    \addplot [black]
    table {%
    2.875 0.0652578713470367
    3.125 0.0652578713470367
    };
    \path [draw=color2, fill=color2]
    (axis cs:3.75,0.0165083714922063)
    --(axis cs:4.25,0.0165083714922063)
    --(axis cs:4.25,0.0473125418048797)
    --(axis cs:3.75,0.0473125418048797)
    --(axis cs:3.75,0.0165083714922063)
    --cycle;
    \addplot [black]
    table {%
    4 0.0165083714922063
    4 -0.00955008071461074
    };
    \addplot [black]
    table {%
    4 0.0473125418048797
    4 0.0775739360156383
    };
    \addplot [black]
    table {%
    3.875 -0.00955008071461074
    4.125 -0.00955008071461074
    };
    \addplot [black]
    table {%
    3.875 0.0775739360156383
    4.125 0.0775739360156383
    };
    \path [draw=color2, fill=color2]
    (axis cs:4.75,0.0140074503267391)
    --(axis cs:5.25,0.0140074503267391)
    --(axis cs:5.25,0.0435504589691983)
    --(axis cs:4.75,0.0435504589691983)
    --(axis cs:4.75,0.0140074503267391)
    --cycle;
    \addplot [black]
    table {%
    5 0.0140074503267391
    5 -0.00908338933413218
    };
    \addplot [black]
    table {%
    5 0.0435504589691983
    5 0.0728768672334231
    };
    \addplot [black]
    table {%
    4.875 -0.00908338933413218
    5.125 -0.00908338933413218
    };
    \addplot [black]
    table {%
    4.875 0.0728768672334231
    5.125 0.0728768672334231
    };
    \path [draw=color2, fill=color2]
    (axis cs:5.75,0.0185436189652562)
    --(axis cs:6.25,0.0185436189652562)
    --(axis cs:6.25,0.0553488337794198)
    --(axis cs:5.75,0.0553488337794198)
    --(axis cs:5.75,0.0185436189652562)
    --cycle;
    \addplot [black]
    table {%
    6 0.0185436189652562
    6 -0.0101918862178658
    };
    \addplot [black]
    table {%
    6 0.0553488337794198
    6 0.0911973347311421
    };
    \addplot [black]
    table {%
    5.875 -0.0101918862178658
    6.125 -0.0101918862178658
    };
    \addplot [black]
    table {%
    5.875 0.0911973347311421
    6.125 0.0911973347311421
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    0.75 0.0165687377359077
    1.25 0.0165687377359077
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    1.75 0.0119685259205868
    2.25 0.0119685259205868
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    2.75 0.0235685435613101
    3.25 0.0235685435613101
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    3.75 0.0295950531683319
    4.25 0.0295950531683319
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    4.75 0.027152738327523
    5.25 0.027152738327523
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    5.75 0.0352274564681333
    6.25 0.0352274564681333
    };
  \end{axis}

\end{tikzpicture}


==> tex/ape_boxplot_adaptive_open_traj.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color5}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color3}{rgb}{0.83, 0.37, 0.00}

  \definecolor{darkslategray38}{RGB}{38,38,38}
  \definecolor{lavender234234242}{RGB}{234,234,242}
  \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
  \definecolor{steelblue76114176}{RGB}{76,114,176}

  \begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    axis background/.style={fill=white},
    axis line style={white},
    tick align=outside,
    x grid style={white},
    xmajorgrids,
    xmajorticks=true,
    xmin=0.5, xmax=6.5,
    % xtick style={draw=none},
    xtick={1,2,3,4,5,6},
    xticklabels={
      \(\displaystyle I_{}^{\text{KF}}\),
      \(\displaystyle I_{\text{AST}}^{\text{KF}}\),
      \(\displaystyle I_{\text{ADT}}^{\text{KF}}\),
      \(\displaystyle I_{}^{\text{EKF}}\),
      \(\displaystyle I_{\text{AST}}^{\text{EKF}}\),
      \(\displaystyle I_{\text{ADT}}^{\text{EKF}}\)
    },
    y grid style={white},
    ylabel=\textcolor{darkslategray38}{Error (m)},
    ymajorgrids,
    ymajorticks=true,
    ymin=-0.016887039108195, ymax=0.0921124627248442,
    % ytick style={draw=none}
    % ytick style={draw=none}
    y grid style={white!69.0196078431373!black},
    ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
    ]
    \path [draw=color3, fill=color3]
    (axis cs:0.75,0.00856180120356441)
    --(axis cs:1.25,0.00856180120356441)
    --(axis cs:1.25,0.0257920654383385)
    --(axis cs:0.75,0.0257920654383385)
    --(axis cs:0.75,0.00856180120356441)
    --cycle;
    \addplot [black]
    table {%
    1 0.00856180120356441
    1 -0.00858209952456189
    };
    \addplot [black]
    table {%
    1 0.0257920654383385
    1 0.0429620472262821
    };
    \addplot [black]
    table {%
    0.875 -0.00858209952456189
    1.125 -0.00858209952456189
    };
    \addplot [black]
    table {%
    0.875 0.0429620472262821
    1.125 0.0429620472262821
    };
    \path [draw=color3, fill=color3]
    (axis cs:1.75,0.00621015506634852)
    --(axis cs:2.25,0.00621015506634852)
    --(axis cs:2.25,0.022808509369406)
    --(axis cs:1.75,0.022808509369406)
    --(axis cs:1.75,0.00621015506634852)
    --cycle;
    \addplot [black]
    table {%
    2 0.00621015506634852
    2 -0.0102993760048189
    };
    \addplot [black]
    table {%
    2 0.022808509369406
    2 0.0393168680048677
    };
    \addplot [black]
    table {%
    1.875 -0.0102993760048189
    2.125 -0.0102993760048189
    };
    \addplot [black]
    table {%
    1.875 0.0393168680048677
    2.125 0.0393168680048677
    };
    \path [draw=color3, fill=color3]
    (axis cs:2.75,0.0205472628126827)
    --(axis cs:3.25,0.0205472628126827)
    --(axis cs:3.25,0.0418105245693556)
    --(axis cs:2.75,0.0418105245693556)
    --(axis cs:2.75,0.0205472628126827)
    --cycle;
    \addplot [black]
    table {%
    3 0.0205472628126827
    3 -0.000715379135904531
    };
    \addplot [black]
    table {%
    3 0.0418105245693556
    3 0.0630732990790338
    };
    \addplot [black]
    table {%
    2.875 -0.000715379135904531
    3.125 -0.000715379135904531
    };
    \addplot [black]
    table {%
    2.875 0.0630732990790338
    3.125 0.0630732990790338
    };
    \path [draw=color3, fill=color3]
    (axis cs:3.75,0.016708325644233)
    --(axis cs:4.25,0.016708325644233)
    --(axis cs:4.25,0.0468532673870428)
    --(axis cs:3.75,0.0468532673870428)
    --(axis cs:3.75,0.016708325644233)
    --cycle;
    \addplot [black]
    table {%
    4 0.016708325644233
    4 -0.010798046206452
    };
    \addplot [black]
    table {%
    4 0.0468532673870428
    4 0.0769731402544181
    };
    \addplot [black]
    table {%
    3.875 -0.010798046206452
    4.125 -0.010798046206452
    };
    \addplot [black]
    table {%
    3.875 0.0769731402544181
    4.125 0.0769731402544181
    };
    \path [draw=color3, fill=color3]
    (axis cs:4.75,0.0149584885436143)
    --(axis cs:5.25,0.0149584885436143)
    --(axis cs:5.25,0.051107141139622)
    --(axis cs:4.75,0.051107141139622)
    --(axis cs:4.75,0.0149584885436143)
    --cycle;
    \addplot [black]
    table {%
    5 0.0149584885436143
    5 -0.0119325162976023
    };
    \addplot [black]
    table {%
    5 0.051107141139622
    5 0.0871579399142515
    };
    \addplot [black]
    table {%
    4.875 -0.0119325162976023
    5.125 -0.0119325162976023
    };
    \addplot [black]
    table {%
    4.875 0.0871579399142515
    5.125 0.0871579399142515
    };
    \path [draw=color3, fill=color3]
    (axis cs:5.75,0.024268365198519)
    --(axis cs:6.25,0.024268365198519)
    --(axis cs:6.25,0.0508873073144224)
    --(axis cs:5.75,0.0508873073144224)
    --(axis cs:5.75,0.024268365198519)
    --cycle;
    \addplot [black]
    table {%
    6 0.024268365198519
    6 -0.00234048248371305
    };
    \addplot [black]
    table {%
    6 0.0508873073144224
    6 0.0773417026044912
    };
    \addplot [black]
    table {%
    5.875 -0.00234048248371305
    6.125 -0.00234048248371305
    };
    \addplot [black]
    table {%
    5.875 0.0773417026044912
    6.125 0.0773417026044912
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    0.75 0.0167478288762138
    1.25 0.0167478288762138
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    1.75 0.0135830949102027
    2.25 0.0135830949102027
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    2.75 0.0317289522588803
    3.25 0.0317289522588803
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    3.75 0.0297950717452046
    4.25 0.0297950717452046
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    4.75 0.0297756960092259
    5.25 0.0297756960092259
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    5.75 0.0376649565098778
    6.25 0.0376649565098778
    };
  \end{axis}

\end{tikzpicture}


==> tex/ape_boxplot_constant.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.39, 0.70, 0.99}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


  \definecolor{darkslategray38}{RGB}{38,38,38}
  \definecolor{lavender234234242}{RGB}{234,234,242}
  \definecolor{mediumseagreen85168104}{RGB}{85,168,104}
  \definecolor{steelblue76114176}{RGB}{76,114,176}

  \begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    axis background/.style={
        % fill=lavender234234242
        draw=white,
    },
    axis line style={white},
    tick align=outside,
    tick pos=left,
    x grid style={white},
    xmajorgrids,
    xmajorticks=true,
    xmin=0.5, xmax=5.5,
    % xtick style={draw=none},
    xtick={1,2,3,4,5,6,7},
    xticklabels={
      \(\displaystyle I_{2}^{}\),
      \(\displaystyle I_{5}^{}\),
      \(\displaystyle I_{10}^{}\),
      \(\displaystyle I_{20}^{}\),
      \(\displaystyle I_{50}^{}\)
    },
    % y grid style={white},
    ylabel=\textcolor{darkslategray38}{Error (m)},
    % ylabel style={yshift=3.5ex},
    ymajorgrids,
    ymajorticks=true,
    % ytick style={draw=none}
    ymin=-0.0194790000970649, ymax=0.135583932449453,
    % ytick style={draw=none}
    y grid style={white!69.0196078431373!black},
    ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
    ]
    \path [draw=color1, fill=color1]
    (axis cs:0.75,0.00589444363535384)
    --(axis cs:1.25,0.00589444363535384)
    --(axis cs:1.25,0.0246149258815733)
    --(axis cs:0.75,0.0246149258815733)
    --(axis cs:0.75,0.00589444363535384)
    --cycle;
    \addplot [black]
    table {%
    1 0.00589444363535384
    1 -0.0120306849813141
    };
    \addplot [black]
    table {%
    1 0.0246149258815733
    1 0.0433309323853461
    };
    \addplot [black]
    table {%
    0.875 -0.0120306849813141
    1.125 -0.0120306849813141
    };
    \addplot [black]
    table {%
    0.875 0.0433309323853461
    1.125 0.0433309323853461
    };
    \path [draw=color1, fill=color1]
    (axis cs:1.75,0.00682313414001156)
    --(axis cs:2.25,0.00682313414001156)
    --(axis cs:2.25,0.0230942986898193)
    --(axis cs:1.75,0.0230942986898193)
    --(axis cs:1.75,0.00682313414001156)
    --cycle;
    \addplot [black]
    table {%
    2 0.00682313414001156
    2 -0.00938493031765407
    };
    \addplot [black]
    table {%
    2 0.0230942986898193
    2 0.039347162699833
    };
    \addplot [black]
    table {%
    1.875 -0.00938493031765407
    2.125 -0.00938493031765407
    };
    \addplot [black]
    table {%
    1.875 0.039347162699833
    2.125 0.039347162699833
    };
    \path [draw=color1, fill=color1]
    (axis cs:2.75,0.0105425014351952)
    --(axis cs:3.25,0.0105425014351952)
    --(axis cs:3.25,0.0288478142860867)
    --(axis cs:2.75,0.0288478142860867)
    --(axis cs:2.75,0.0105425014351952)
    --cycle;
    \addplot [black]
    table {%
    3 0.0105425014351952
    3 -0.00775220779928957
    };
    \addplot [black]
    table {%
    3 0.0288478142860867
    3 0.047131058002699
    };
    \addplot [black]
    table {%
    2.875 -0.00775220779928957
    3.125 -0.00775220779928957
    };
    \addplot [black]
    table {%
    2.875 0.047131058002699
    3.125 0.047131058002699
    };
    \path [draw=color1, fill=color1]
    (axis cs:3.75,0.0201896099672381)
    --(axis cs:4.25,0.0201896099672381)
    --(axis cs:4.25,0.042625070862684)
    --(axis cs:3.75,0.042625070862684)
    --(axis cs:3.75,0.0201896099672381)
    --cycle;
    \addplot [black]
    table {%
    4 0.0201896099672381
    4 -0.00223572135256648
    };
    \addplot [black]
    table {%
    4 0.042625070862684
    4 0.0650276111353747
    };
    \addplot [black]
    table {%
    3.875 -0.00223572135256648
    4.125 -0.00223572135256648
    };
    \addplot [black]
    table {%
    3.875 0.0650276111353747
    4.125 0.0650276111353747
    };
    \path [draw=color1, fill=color1]
    (axis cs:4.75,0.0386564688920522)
    --(axis cs:5.25,0.0386564688920522)
    --(axis cs:5.25,0.0734428699045647)
    --(axis cs:4.75,0.0734428699045647)
    --(axis cs:4.75,0.0386564688920522)
    --cycle;
    \addplot [black]
    table {%
    5 0.0386564688920522
    5 0.00392419819438428
    };
    \addplot [black]
    table {%
    5 0.0734428699045647
    5 0.108144410137385
    };
    \addplot [black]
    table {%
    4.875 0.00392419819438428
    5.125 0.00392419819438428
    };
    \addplot [black]
    table {%
    4.875 0.108144410137385
    5.125 0.108144410137385
    };
    \path [draw=color1, fill=color1]
    (axis cs:5.75,0.0300148168482776)
    --(axis cs:6.25,0.0300148168482776)
    --(axis cs:6.25,0.0835341570252374)
    --(axis cs:5.75,0.0835341570252374)
    --(axis cs:5.75,0.0300148168482776)
    --cycle;
    \addplot [black]
    table {%
    6 0.0300148168482776
    6 -0.0112948643904059
    };
    \addplot [black]
    table {%
    6 0.0835341570252374
    6 0.136935617333703
    };
    \addplot [black]
    table {%
    5.875 -0.0112948643904059
    6.125 -0.0112948643904059
    };
    \addplot [black]
    table {%
    5.875 0.136935617333703
    6.125 0.136935617333703
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    0.75 0.0134189554989298
    1.25 0.0134189554989298
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    1.75 0.0142722262942559
    2.25 0.0142722262942559
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    2.75 0.0184918652005616
    3.25 0.0184918652005616
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    3.75 0.0306511992622468
    4.25 0.0306511992622468
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    4.75 0.0552353236831163
    5.25 0.0552353236831163
    };
    \addplot [line width=1pt, white, forget plot]
    table {%
    5.75 0.0508436389209047
    6.25 0.0508436389209047
    };
  \end{axis}

\end{tikzpicture}

